The Resolved NIR Extragalactic Background

We present a current best estimate of the integrated near-infrared (NIR) extragalactic background light (EBL) attributable to resolved galaxies in J, H, and Ks . Our results for measurements of {\nu}I{\nu} in units of nW m-2 sr-1 are 11.7+5.6 -2.6 in J, 11.5+4 .5 -1.5 in H and 10.0+2 .8 -0.8 in Ks . We derive these new limits by combining our deep wide-field NIR photometry from five widely separated fields with other studies from the literature to create a galaxy counts sample that is highly complete and has good counting statistics out to J H Ks ~ 27 - 28. As part of this effort we present new ultradeep Ks -band galaxy counts from 22 hours of observations with the Multi Object Infrared Camera and Spectrograph (MOIRCS) instrument on the Subaru Telescope. We use this MOIRCS Ks -band mosaic to estimate the total missing flux from sources beyond our detection limits. Our new lim- its to the NIR EBL are in basic agreement with, but 10 - 20% higher than previous estimates, bringing them into better agreement with estimates of the total NIR EBL (resolved + unresolved sources) obtained from TeV {\gamma}-ray opacity measurements and recent direct measurements of the total NIR EBL, as well as recent model estimates for the total light from galaxies. We exam- ine field to field variations in our photometry to show that the integrated light from galaxies is isotropic to within uncertainties, consistent with the expected large-scale isotropy of the EBL.

==> Table1.tex <==
\begin{deluxetable*}{ccccccc}
\tablecaption{\label{avgcntstab}Average Galaxy Counts Used to Calculate the NIR EBL}
\tablehead{  & \multicolumn{2}{c}{~~~$J$~~~} &\multicolumn{2}{c}{~~~$H$~~~} & \multicolumn{2}{c}{~~~$K_s$~~~}}  
\startdata
Mag(AB)\tablenotemark{a}  & Log$_{10}$($N$)\tablenotemark{b} & Log$_{10}$($\Delta N$)\tablenotemark{c} & Log$_{10}$($N$)  & Log$_{10}$($\Delta N$) &  Log$_{10}$($N$)  & Log$_{10}$($\Delta N$)  \\
\hline
11&-1.31&-2.33&-1.13&-2.67&-1.27&-2.76  \\
12&-0.67&-2.10&-0.51&-2.02&-0.63&-1.94  \\
13&-0.06&-1.27&0.089&-1.60&-0.01&-1.64  \\
14&0.500&-1.30&0.660&-0.25&0.603&-0.92  \\
15&1.084&0.121&1.262&-0.32&1.229&0.553  \\
16&1.654&0.726&1.842&1.004&1.891&0.379  \\
17&2.290&1.517&2.425&1.519&2.592&2.013  \\
18&2.910&2.365&3.030&1.786&3.149&1.851  \\
19&3.340&2.665&3.453&2.644&3.554&2.228  \\
20&3.713&3.117&3.825&2.736&3.901&2.479  \\
21&4.098&3.495&4.148&3.368&4.200&2.701  \\
22&4.455&3.811&4.488&3.476&4.459&2.946  \\
23&4.719&4.162&4.781&4.059&4.795&3.669  \\
24&4.916&4.391&4.965&4.170&5.008&3.931  \\
25&5.067&4.242&5.156&4.732&5.178&4.653  \\
26&5.285&4.439&5.297&4.647&5.324&4.618  \\
27&5.370&4.297&5.361&5.055&5.462&5.227  \\
28&5.376&4.717&5.456&4.755&5.547&4.983  \\
\enddata
\tablenotetext{a}{AB Magnitude.}
\tablenotetext{b}{$N$ is the surface density of galaxies in units of $\rm{mag}^{-1}\rm{deg}^{-2}$.}
\tablenotetext{c}{$\Delta N$ is the $1~\sigma$ error estimate for N (in
  the same units) derived from
  the fits described in Section~\ref{nir_resolved} to all the data shown in Figure~\ref{mycounts}.}
\end{deluxetable*}


==> Table2.tex <==
\begin{deluxetable*}{llll}
\tablewidth{0pt}
\tabletypesize{\scriptsize}
\tablecaption{\label{nirebl_tab}NIR Integrated Galaxy Light ($\nu I_{\nu};~\rm{nW}~\rm{m}^{-2}~\rm{sr}^{-1}$)}
\tablehead{ ~~~~~& $J$\tablenotemark{a} & $H$ & $K_s$\tablenotemark{b}} 
\startdata
\scriptsize{This work}\tablenotemark{c} & 11.7~(+3)~$\pm 2.6$&11.5~(+3)~$\pm
1.5$&10.0~(+1.9)~$\pm 0.8$\\
\scriptsize{\citet{Mada00}}& $9.7^{\tiny{+3.0}}_{\tiny{-1.9}}$ & $9.0^{\tiny{+2.6}}_{\tiny{-1.7}}$ & $7.9^{\tiny{+2.0}}_{\tiny{-1.2}}$  \\
\scriptsize{\citet{Tota01}}& $10.9~\pm~1.1$ & N/A & $8.3~\pm~0.8$ \\
\scriptsize{\citet{Thom03}\tablenotemark{d}}& N/A & 7.0 & N/A \\
\enddata
\tablenotetext{a}{\citet{Mada00} $J-$band is centered at $1.1 \mu$m while this and other studies listed are centered at $1.25~\mu$m.}
\tablenotetext{b}{This work is done at $K_s (2.12~\mu$m) while \citet{Mada00} and \citet{Tota01} are at $K (2.2~\mu$m).}
\tablenotetext{c}{Missing flux estimates are given in parentheses next to our
  measured values for the IGL.  The missing flux in the $J$ and $H-$bands are
  taken from \citet{Thom07a} and for $K_s-$band the value is derived as
  described in Section~\ref{missingflux}.  The confidence intervals given are
  the $1~\sigma$ error estimates from the galaxy counts fits described in Section~\ref{nir_resolved}.}
\tablenotetext{d}{$\rm{Lower~limit}$.}
\end{deluxetable*}

